Optimizing Long-tailed Link Prediction in Graph Neural Networks through Structure Representation Enhancement

Link prediction, as a fundamental task for graph neural networks (GNNs), has boasted significant progress in varied domains. Its success is typically influenced by the expressive power of node representation, but recent developments reveal the inferior performance of low-degree nodes owing to their sparse neighbor connections, known as the degree-based long-tailed problem. Will the degree-based long-tailed distribution similarly constrain the efficacy of GNNs on link prediction? Unexpectedly, our study reveals that only a mild correlation exists between node degree and predictive accuracy, and more importantly, the number of common neighbors between node pairs exhibits a strong correlation with accuracy. Considering node pairs with less common neighbors, i.e., tail node pairs, make up a substantial fraction of the dataset but achieve worse performance, we propose that link prediction also faces the long-tailed problem. Therefore, link prediction of GNNs is greatly hindered by the tail node pairs. After knowing the weakness of link prediction, a natural question is how can we eliminate the negative effects of the skewed long-tailed distribution on common neighbors so as to improve the performance of link prediction? Towards this end, we introduce our long-tailed framework (LTLP), which is designed to enhance the performance of tail node pairs on link prediction by increasing common neighbors. Two key modules in LTLP respectively supplement high-quality edges for tail node pairs and enforce representational alignment between head and tail node pairs within the same category, thereby improving the performance of tail node pairs.

==> del3-preliminary.tex <==
\section{preliminary}


Given an undirected graph $\mathcal{G} = \left(\mathcal{V},\mathcal{E} \right)$ consisting of the node set $\mathcal{V} = \{v_1,v_2,v_3,\dots,v_N \}$ and the edge set $\mathcal{E}$. Commonly, each edge $e_{u,v}$ in the edge set $\mathcal{E}$ denotes the connection between node $v_u$ and $v_v$, and each node $v$ within $\mathcal{G}$ has its own feature vector $\bm{x}_v \in \mathbb{R}^f$ with f-dimension.
Graph Neural Networks (GNNs) learn node representation by leveraging an iterative aggregation function to harness the information from neighbors. The representation of node $v$ at the $l-th$ layer can be articulated as follows:
\begin{equation}
    \bm{h}_{v}^{(l)} = \sigma (\bm{h}_{v}^{(l-1)}, \phi (\{\bm{h}_{u}^{(l-1)} | u \in \mathcal{N}_{v} \}) ),
\end{equation}
where $\sigma(\cdot)$ combines the representation of node $v$ and its neighbors $\mathcal{N}_v$ in the $l-th$ layer, $\phi(\cdot)$ is the aggregation function such as GCN, GAT, etc. Meanwhile, we set $\bm{h}_{v}^{0}=\bm{x}_v $ as the initialization state.

Link prediction aims to learn the prediction function $\mathcal{F}(u,v|\mathcal{G})$ to estimate the likelihood of whether there is a connection between the target node pair $(u, v)$, and the formulation of node pair $(u,v)$ after $L$ layers can be expressed as:
\begin{equation}
    \mathcal{F}(u,v|\mathcal{G}) = \textit{f} ( \psi (\bm{h}_{v}^{(L)}, \bm{h}_{u}^{(L)}) ),
\end{equation}
where $\psi(\cdot)$ can take the form of an inner product or a multi-layer MLP and then map to $[0,1]$ using $\textit{f}(\cdot)$. 

Additionally, several link prediction approaches have made significant strides by learning from subgraph $\mathcal{G}_{u,v}$, such as SEAL, Grail, Neo-GNN, and NBFNet. These approaches enhance performance by extracting information from subgraphs $\mathcal{G}_{u,v}$ formed between target nodes $(u,v)$. The formulation in these schemes can be redefined as follows:
\begin{equation}
    \mathcal{F}(u,v|\mathcal{G}_{u,v}) = \textit{f} ( \psi (\bm{h}_{v}^{(L)}, \bm{h}_{u}^{(L)}) ),
\end{equation}
where $\bm{h}_{v}^{(L)}$ and $\bm{h}_{u}^{(L)}$ here are also benefit from the subgraph $\mathcal{G}_{u,v}$.



Having formalized the link prediction function $\mathcal{F}(u,v|\mathcal{G})$, we proceed to optimize the model parameters $\theta$ with loss function $\mathcal{L}(\cdot)$ as follows :
\begin{equation}
    \min_{\theta} =\sum_{(u, v, y_{u,v}) \in \mathcal{O}}{\mathcal{L}(\mathcal{F}(u, v|\mathcal{G}), y_{u, v})},
\end{equation}
where $\mathcal{O}$ is the training set defined by node pair $(u,v)$ and their labels $y_{u, v}$ where we set $y_{u, v}=1$ if edge $e_{u,v}$ is in the edge set $\mathcal{E}$, otherwise as 0. $\mathcal{L}(\cdot)$ is defined as cross-entropy function in most link prediction works such as seal and neo-gnn. 





% Link prediction tasks aim to learn the prediction function $\mathcal{F}(u,v|\mathcal{G}; \theta)$ to estimate the likelihood of whether there is a connection between the target node pair $(u, v)$, which commonly involves an encoder and a decoder component. 

% In the realm of graph-based learning, encoders are employed to characterize nodes utilizing the information from their neighbors. Given the potent expressive power of Graph Neural Networks (GNNs), the majority of contemporary models harness GNNs as encoders. The formalization of such models is as follows:

% \paratitle{Encoder}
% In terms of link prediction, the encoder is utilized to generate node representations by leveraging the neighboring data. The advent of graph neural networks (GNNs) has positioned them as a preferred choice for encoding, which recursively aggregate and update representations based on neighborhood information across the entire graph (i.e. $\mathcal{G}$). Specifically, we detail the iterative process of a GNN for a node $v$ as follows:


% \begin{equation}
%     \begin{split}
%         \bm{h}^{(l+1)}_{v} & = \textit{Encoder}(\bm{h}_v^{(l)}|\mathcal{G}; \theta^{\mathcal{G}}) \\
%                            & = \textit{UPD}(\bm{h}_v^{(l)}, \textit{AGG}(\bm{h}_{v'}^{(l)}|{v' \in \mathcal{N}_v}; \theta^{\mathcal{G}, \mathcal{A}}); \theta^{\mathcal{G}, \mathcal{U}}), \\
%     \end{split}
% \end{equation}
% where $\bm{h}_v^{(l)}, \bm{h}_v^{(l+1)}$ respectively denote the node representations as the $l$ and $l+1$-th layer, and $\bm{h}_v^{(0)}$ is initialized with its original feature vector $\bm{x}_v$, and $\mathcal{N}_{v}$ represent the neighbors of node $v$. Here, $\textit{Encoder}(\cdot)$ is formally parameterized by $\theta^{\mathcal{G}}$, which, in particular, is comprised of the $\theta^{\mathcal{G}, \mathcal{A}}$-parameterized aggregation function $\textit{AGG}(\cdot)$ and $\theta^{\mathcal{G}, \mathcal{U}}$-parameterized updating function  $\textit{UPD}(\cdot)$.
% As the core of GNNs, several efforts have been made towards the design of the aggregation and updating function~\cite{gat,geniepath}.
% Additionally, edge-centric link prediction approaches have made significant strides, such as SEAL, Grail, Neo-GNN, and NBFNet. These approaches enhance performance by extracting information from subgraphs $\mathcal{G}_{u,v}$ formed between target nodes $(u,v)$. The encoder in these schemes can be reformulated as $\text{Encoder}(\bm{h}_v | \mathcal{G}_{u,v}; \theta^{\mathcal{G}})$.


% \paratitle{Decoder}
% After $L$-layers iterations, the decoder is used to splice the final representations (i.e. $\bm{h}^{(L)}_{u},\bm{h}^{(L)}_{v}$) for each node pair $(u, v)$ and make a prediction. The decoder is formalized as follows: 
% \begin{equation}
%     \textit{Decoder}(u,v|\mathbf{H}; \theta^{\mathcal{P}}) = \sigma(\bm{h}^{(L)}_{u}, \bm{h}^{(L)}_{v}; \theta^{\mathcal{P}}),
% \end{equation}
% where $\mathbf{H} \in \mathbb{R}^{|\mathcal{V}| \times d}$ is the collection of graph’s learned node representations with $d$-dimension in a matrix form.  $\sigma(\cdot)$ can take the form of inner product or a multi-layer MLP. In our case, $\sigma(\cdot)$ is implemented as the inner product. 

% Having formalized the link prediction function $\mathcal{F}(u,v|\mathcal{G}; \theta)$, we proceed to optimize parameters $\theta$ with loss function $\mathcal{L}(\cdot)$ as follows :
% \begin{equation}
%     \min_{\theta} =\sum_{(u, v, y_{u,v}) \in \mathcal{O}_{train}}{\mathcal{L}(\mathcal{F}(u, v|\mathcal{G}; \theta), y_{u, v})},
% \end{equation}
% where $\mathcal{O}_{train}$ is the training data, $\mathcal{L}(\cdot)$ is defined as cross-entropy function in seal and neo-gnn. if node pair $(u,v)$ is present in the edge set $\mathcal{E}$, which indicate it has been observed, we define $y_{u, v}$ as 1, otherwise as 0. 



